Computational Network Design from Functional Specifications

Connectivity and layout of underlying networks largely determine the behavior of many environments. For example, transportation networks determine the flow of traffic in cities, or maps determine the difficulty and flow in games. Designing such networks from scratch is challenging as even local network changes can have large global effects. We investigate how to computationally create networks starting from {\em only} high-level functional specifications. Such specifications can be in the form of network density, travel time versus network length, traffic type, destination locations, etc. We propose an integer programming-based approach that guarantees that the resultant networks are valid by fulfilling all specified hard constraints, and score favorably in terms of the objective function. We evaluate our algorithm in three different design settings (i.e., street layout, floorplanning, and game level design) and demonstrate, for the first time, that diverse networks can emerge purely from high-level functional specifications.

==> guidelines.tex <==
 \section{Street Network Design Guidelines}
 \label{sec:guidelines}








The purpose of street networks is to connect one place to another. However, the process is complicated by various conflicting requirements. For example, it is desirable to have
short commute times among places. This, on the other hand, encourages a densely connected network, which can be less attractive for residential neighborhoods (see Figure~\ref{fig:guideline}).
Manually balancing between such global and local considerations is difficult, and hence street design for urban planning remains a task requiring specialized skill and knowledge.
%
We studied commonly used design practices from the relevant literature~\cite{Southworth:1995:SSA,Meyer:00,Southworth03,planStreet:03,APA:06,TRB:2010:HCM,Ortuzar:11,Marshall:2011:SP}. From these works, we recommend the standards guideline~\cite{APA:06} for a simple introduction to urban planning in general and~\cite{Ortuzar:11} for a more technical introduction to transportation models. We extracted three key design guidelines from the literature as described next.


% (c.f.,~\cite{xx,yy,}) and .
%, which we later utilize in our computational framework. First, we describe the guidelines.


% Streets and Patterns \cite{Marshall:2011:SP}
% Street standards and the shaping of suburbia \cite{}
% Streets and the Shaping of Towns and Cities \cite{}
% The Architectural Pattern Book: A Tool for Building Great Neighborhoods \cite{Robinson04}
% Planning and urban design standards \cite{APA:06}
% Urban Transportation Planning \cite{Meyer:00}
% Modelling Transport \cite{Ortuzar:11}
%Highway Capacity Manual \cite{TRB:2010:HCM}



\mypara{Hierarchical layout} Urban street networks are typically designed hierarchically. High speed {\em principal} and {\em minor arterial streets} are first distributed at regular spacing (typically 3 miles and 1 mile intervals, respectively) to carry
bulk of the traffic. Residential blocks are then linked to such arterial networks by slower but densely spaced {\em collector streets}; and finally local traffic is allowed inside individual residential blocks through {\em local streets}. Note that,
by enforcing speed restrictions on the denser streets (i.e., collectors and  locals), though traffic is discouraged (and in some cases prohibited), which in turn ensures that the coarse arterial street networks chiefly determine the global traffic flow pattern.


\mypara{Street connectivity} At a local level, street connectivity and speed limits play important roles in determining travel patterns and connectivity. For example, by controlling direct and indirect connections in a neighborhood (e.g., residential block), planners
can provide high connectivity or quieter cul-de-sacs (see Figure~\ref{fig:guideline}).
%
Commonly used layout styles follow grid, grid and diagonal, web, radial, or simply irregular patterns.
%
Note that as a secondary effect, the choice of extent of blocks and their connectivity can also determine if an individual will travel to her destination, or simply walk or bike. (We do not consider this effect in our work).
%
Usually local access is measured by the {\em connectivity index}, which is the ratio of the number of links (i.e., streets) to the number of nodes (i.e., intersections) in the network.
%
While higher connectivity index indicate higher network redundancy. %, most cities require the minimum value to be in the range 1.2 to 1.4.




\mypara{Block parceling} Street networks implicitly partition urban landscapes into blocks (e.g., residential or commercial), which are in turn split to create parcels, e.g., building footage and landscapes.
%
Not surprisingly, the parceling of blocks has immediate socioeconomic implications.
%
For example, sparse street networks not only leave more usable block space, but can encourage larger, expensive, and well-spaced parcel layouts.
%
However, although various block types (e.g., square, organic, elongated, mixed) are commonly used, they can mostly be derived by offsetting  or skeletonizing the street networks and indicating local parcel density.






%limitations: dont consider redundant connections; walk vs. bike; effect of terrain 

==> methodology.tex <==
\section{Methodology}
\label{sec:methodology}

We propose an algorithm to generate street networks starting only from functional specifications.
%
The user indicates the total working boundary and provides high level goals like traffic flow (e.g., fast or slow)  and street usage (e.g., busy, quiet) along certain directions (e.g., vertical, horizontal, diagonal), and block quality (e.g., access to interior of the blocks).
%
Based on these, we design a street network, i.e., topology of the network, its geometric layout, and also associated parcel specification.
%
The problem is challenging as there is a strong coupling: in order to determine travel times, we need information about the network layout (both its connectivity and geometry); however, the network is unknown and only indirectly indicated via qualitative functional specifications involving target travel time, block properties, etc.
Further, we start from scratch without guidance from pre-authored template layouts.
Even a simple baseline solution is hard to think of since one cannot possibly evaluate all possible street layouts. Also, we need to characterize what makes desirable street networks.


Inspired by the guidelines summarized in Section~\ref{sec:guidelines}, we propose an algorithm that runs in three key stages (see Figure~\ref{fig:algo_stages}): first, {\em global optimization} to obtain a coarse network flow based on the target functional specifications; then, {\em local geometry layout} to realize the coarse network by working out specific street connectivity and local geometry; and finally {\em parcel generation} to divide the building areas (i.e., not covered by streets) into individual parcel specifications and provide necessary connectivity to the street network.
%
A key aspect of the algorithm is the global-local separation, which allows designing a coarse network behavior {\em without} committing to its specific geometric realization.



\begin{figure}[b!]
   \vnudge
  \begin{overpic}[width=\columnwidth]{figures/real_layout/real_layout.pdf}
  \put(5,5){$\mathbf{M}^{1,1}$}
  \put(16.5,5){$\mathbf{M}^{1,2}$}
  \put(28,5){$\mathbf{M}^{1,3}$}
  \put(5,17){$\mathbf{M}^{2,1}$}
  \put(16.5,17){$\mathbf{M}^{2,2}$}
  \put(28,17){$\mathbf{M}^{2,3}$}
  \put(5,28){$\mathbf{M}^{3,1}$}
  \put(16.5,28){$\mathbf{M}^{3,2}$}
  \put(28,28){$\mathbf{M}^{3,3}$}
  %
  \put(56,1.5){$\mathbf{M}^{2,2}$}
  \end{overpic}
   \caption{In the global optimization stage, we first optimize for a coarse network
   to satisfy the input functional specifications.
   The specified boundary (in orange), is first split into a regular $m \times n$ grid. Neighboring grid cells can be connected via connectors (in green circles). The network is then
   modeled as a set of connectivity matrices, each being a $4 \times 4$ matrix. Entries in the matrices denote the travel time between the corresponding elements, e.g., $\mathbf{M}^{2,2}_{a,c}$ captures that the commute time $a \rightarrow c$ is 4 time units.
   Since we allow travel times to be different in opposite directions, note that the matrices are not necessarily symmetric.  }
   \label{fig:global_matrix}
\end{figure}

%
We partition a given map boundary into a grid, say an $m \times n$ regular grid.
Intra- and inter-cell links are provided by connectors (see Figure~\ref{fig:global_matrix}).
%
We assume a single connector between each pair of neighboring cells and hence four connectors for each cell.
%
Inside the $(i,j)$-th cell, we consider all possible six connections and encode their flow behavior as a {\em connectivity matrix} $\mathbf{M}^{i,j}_{4 \times 4}$. Entries of such a matrix indicate the estimated travel time between the corresponding connectors.
Note that the matrix is not necessarily symmetric since we allow opposite directions to possibly have different travel times.
If there is no direct link between two connectors, the corresponding matrix entry is set to $\infty$.
%
Starting from functional specifications, in the global optimization phase, we
build a set of connectivity matrices $\{\mathbf{M}^{i,j}\}$ (there are $m \times n$ such matrices). Note that there are $12mn$ unknowns (i.e., connection links) in specification of the coarse network.
Then, in the geometry layout phase, we realize $\{\mathbf{M}^{i,j}\}$ as a local map; and finally, in the parcel generation phase,
design parcel layout and access pattern for the local map. We now describe the steps in details.





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Global Optimization}
\label{subsec:globalOpt}


In this stage, we use high-level functional specifications to build connectivity matrices $\{\mathbf{M}^{i,j}\}$. We first define street network measures (i.e., energies) as a function of the (unknown) matrix entries to quantify travel time, street usage, and street access. Then, we optimize for a coarse network to achieve the target behavior by addressing two tasks: determining which grid cells should be connected; and if connected, how fast the (directional) connection link should be.
%
We achieve this by alternating between a discrete step to determine if a link exists or not; and a continuous step to improve the network behavior while keeping the connectivity fixed.
%
We first describe the energy choices.



\mypara{Street network measures} We consider three energy measures, which often conflict each other and hence require a design tradeoff.

{\em (i)~Travel time:}
Generally, we would like to minimize travel time, but we need to trade off travel time to achieve other goals (e.g., have low trough traffic on residential roads). The user can additionally indicate the directional traffic that is to be measured, along with traffic conditions.

Users have access to the following options for functional specification (one or multiple specifications): traffic direction (e.g., horizontal, vertical, diagonal), speed (e.g., fast or slow), and region specific importance as weights. Note that users can only indicate source/sink at the level of the grid cells. Typical options include from inside to inside cells, from left boundary to right boundary, from boundary to center, etc. The user can optionally specify which source/sink to consider.


\begin{figure}[t!]
  \begin{overpic}[width=\columnwidth]{figures/real_layout/shortest_path.pdf}
  \put(7,60){$t_1$}
  \put(10,51){$t_2$}
  \put(10,46){$t_3$}
  \put(7,37){$t_4$}
  %
  \put(18.5,60){$t_5$}
  \put(21,51){$t_6$}
  \put(21,46){$t_7$}
  \put(18.5,37){$t_8$}
  %
  \put(31,61){$t_9$}
  \put(26,57){$t_{10}$}
  \put(31,46){$t_{11}$}
  \put(29,37){$t_{12}$}
  %
  \put(7,28.5){$a'$}
  \put(7,67.5){$a$}
  \put(19,28.5){$b'$}
  \put(20,67.5){$b$}
  \put(30,28.5){$c'$}
  \put(30,67.5){$c$}
  %
  \put(50,60){$\mathbf{R}^{a\rightarrow a'}=\{t_1,t_2,t_3,t_4\}$}
  \put(50,50){$\mathbf{R}^{b\rightarrow b'}=\{t_5,t_6,t_7,t_8\}$}
  \put(50,40){$\mathbf{R}^{c\rightarrow c'}=\{t_9,t_{10},t_6,t_{11},t_{12}\}$}
  \end{overpic}
   \caption{We measure performance of any coarse network based on its (unknown) connectivity encoded as $\{\mathbf{M}^{i,j}\}$. (Top)~In this example, with the current state of connectivity,
   the unknowns are $t_1,\dots,t_{12}$. Given the specified traffic direction, vertical in this example, we investigate traffic along $\mathbf{R}^{a\rightarrow a'}, \mathbf{R}^{b\rightarrow b'}$, etc.
   We measure travel time, street usage, and street access. In this example, for the three routes, all links have single usage, except for $t_6$, which has usage as 2. Note that as illustration we show a
   particular connectivity; in practice, our algorithm also searches over unknown connectivity.
   %
   (Bottom)~Usage values for different traffics are shown for the result presented in Figure~\protect\ref{fig:algo_stages}.
   }
   \label{fig:grid_connection}
   \vnudge
\end{figure}



Travel time energies, however, are closely linked to the routes chosen between source/sink points. We consider shortest paths between connectors and compute them using Dijkstra's algorithm (one could instead use Floyd-Warshall algorithm) using the current connectivity graph and link values. (We also optimize over connectivity as explained later.)
%
We encode the $k$-th such route $\mathbf{R}^k$ between source/sink points as a series of edges (computed using Dijkstra's algorithm) as $\mathbf{R}^k := \{R^k_{1}, R^k_{2}, \dots,\}$ and having weight $w_k$. (By default weights are set to one.)
Let $t(R^k_{l})$ denote the time it takes to travel along link  $R^k_{l}$.
%
For example, in Figure~\ref{fig:grid_connection}, $\mathbf{R}^{a\rightarrow a'}$ denotes one such route with corresponding (variable) travel times being $\{t_1,t_2,t_3,t_4\}$ (where we used $t_i$ to denote both link and link values for convenience).
%
The average travel time across any such network with $N$ number of routes is then estimated as:
%
\begin{equation}
T(\{\mathbf{M}^{i,j}\}) :=  {\sum_{k=1}^N {\sum_{l} w_k {t(R^k_{l})}} } / {\sum_{k=1}^N {w_k}}
\label{eq:tot_travel}
\end{equation}
as a function of the (unknown) edge link values (i.e., entries of the connectivity matrices).

We measure travel time options as, \\
(a)~{\em fast}
$E_T(\{\mathbf{M}^{i,j}\}) := {T}/{T_0}$ and \\
(b)~{\em slow} $E_T(\{\mathbf{M}^{i,j}\}) := 1 - {T}/{T_0}$, \\
with $T_0$ being a normalization constant set as the estimated maximum travel time. (For simplicity, we use the same notation for the two $E_T$-s.)
Note that users can select different options (i.e., fast/slow) along different routes (see Section~\ref{sec:results}).


{\em (ii)~Street usage:} Typically, we want low street usage in residential areas, i.e., fewer routes sharing the same connection link. However, not all regions can have low usage as that leads to large travel times across the network (in absence of sufficient coverage).
%
By usage of a connection link, we simply measure how many routes pass through it.
Note that the usage of a link is exactly its corresponding coefficient in Equation~\ref{eq:tot_travel}.
Let, $u_k$ denote the usage for the $k$-th link. For example, usage of $t_6$ is 2 in Figure~\ref{fig:grid_connection} for vertical routes.

%
We provide three basic functional specifications to measure usage: \\
(a)~{\em maximum usage} as $E_U(\{\mathbf{M}^{i,j}\}) := \max_k{u_k}$; \\
(b)~{\em inside-periphery} ratio as the fractional usage by streets inside the map compared to the whole map (which also contains the streets on the boundary)
$E_U(\{\mathbf{M}^{i,j}\}) :=  {\sum_{inside} {u_k}} / {\sum_{all} {u_k}}$; and \\
(c)~{\em busyness} as the fraction of connection links above certain usage threshold (i.e., too noisy) as $E_U(\{\mathbf{M}^{i,j}\}) :=   {\#(u_k > threshold)}/ {\#(u_k)}$.

Users can select among these options. Note that the usage terms are also weighted based on route importance (but left out to simplify notation).


{\em (iii)~Street access:}
%
Access roads (see Section~\ref{fig:guideline}) provide easy passage from buildings to the streets. Such roads, however, reduce the amount of available area for buildings.  The user can also functionally specify the target ratio. We measure
access just by scaling (by $\alpha$) the number of active links. The user can either measure access energy as: \\
(a)~$E_A(\{\mathbf{M}^{i,j}\}) :=  \#(M_{k,l}^{i,j}|M_{k,l}^{i,j}<\infty,k!=l)\alpha$, or \\       %   \#(t(M_{k,l}^{i,j}|k\ne l) | t(M_{k,l}^{i,j}|k\ne l) < \infty ) \alpha $, or \\   %    R^k_l)| t(R^k_l) < \infty
(b)~a deviation from an indicated threshold $\Gamma$ as $E_A(\{\mathbf{M}^{i,j}\}) := | \#(M_{k,l}^{i,j}|M_{k,l}^{i,j}<\infty,k!=l)\alpha - \Gamma|$.

The total energy in terms of the connectivity matrices is then defined as:
\begin{equation}
\small
E_{tot}(\{\mathbf{M}^{i,j}\}) := a_1 E_T(\{\mathbf{M}^{i,j}\}) + a_2 E_U(\{\mathbf{M}^{i,j}\}) + a_3 E_A(\{\mathbf{M}^{i,j}\})
\label{eq:optFunction}
\end{equation}
where, ${a_1, a_2, a_3}$ are relative weights.
(Energies $E_T$ and $E_U$ can be a summation of terms if multiple functional specifications are specified.)
Note that lower energy values indicate more desirable layouts.





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\mypara{Mixed Optimization} We minimize Equation~\ref{eq:optFunction} by alternately performing discrete topology optimization and continuous optimization, as explained next.

{\em Topology optimization:}
In this step, we use simulated annealing~\cite{Kirkpatrick:83} to change the connectivity of the network. The main purpose of this stage is to allow connectivity changes, i.e., toggling (random) entries of the matrix between $\infty$ or a positive value. The actual values for the active links are later refined in the continuous optimization step.

Each entry of the connectivity matrices (except the $0$s on the diagonal) can be either a positive value (i.e., travel time from one connector to connector), or be $\infty$ (i.e., no direct link between the connectors). We call the connectivity of the cells sides as topology.

In this stage, the algorithm can change the connectivity between two connectors, with the restriction that certain connective combination within a cell are disallowed (e.g., it results in a matrix that is not realizable in the next stage), or other global constraints (e.g., masked area for park or shop, or make sure enough accessibility for all residential area, etc.). (We would release source code for online implementation details of these constraints.)



\begin{figure}[t!]
   \includegraphics[width=\columnwidth]{figures/energy_effect/energy_iso.pdf}
   \caption{Effect of relative weights $(a_1, a_2, a_3)$ in $E_{tot}$. From left to right: (0.65,0.15,0.2); (0.8,0.1,0.1); (0.78,0.1,0.02); and (0.1,0.8,0.1). }
   \label{fig:eneergy_balance}
   \vnudge
\end{figure}


Moreover, we do not want to have any island in the map, i.e., any road segment that is not connected to the boundary.
Hence, when we disconnect any connection, the algorithm checks the presence of an island; similarly, when we add a new connection, the algorithm verifies that the new connection is not a new island.
%
%
%%% About test island
%Specifically, to test for islands we have two possible conditions:
%(i)~If a new connection is added, test if either of its connectors connecting to any other connections. If not, the new connection is a new island.
%(ii)~If an old connection is removed, test both connectors as follows. Traverse the map from that connector in a breadth first order. If either reaches a connector on the boundary, it is not an island.

%%%% More explanation
In each step of simulated annealing, the algorithm randomly chooses a potential connection and toggles its connectivity.
First, the algorithm tests the validity of the new map with respect to constraints (coverage, mask, etc.) and island check.
If valid, we calculate a new energy from this map, compare with the old energy, and decide whether to accept this change based on the annealing temperature.


%We use simulated annealing to optimize the topology.
Note that we perform simulated annealing until convergence, but only a few iterations each time (about 10 in our tests). The actual parameter refinement happens next when we switch to the continuous optimization.



{\em Continuous optimization:}
While keeping the topology fixed, we now improve the network parameters using a gradient descent method. Given our energy formulation (see Equation~\ref{eq:optFunction}) we can compute the gradients in closed form. For example, in case of fast $E_T$ energy, entries of
$\nabla E_{tot}(\{\mathbf{M}^{i,j}\})$ take the form,
\begin{equation}
\frac {\partial E_{tot}(\{\mathbf{M}^{i,j}\})}{\partial t_l} =
a_1 \frac {\partial E_T(\{\mathbf{M}^{i,j}\})}{\partial t_l} = \frac{a_1}{T_0} u_l
\end{equation}
for any link $t_l$ and $u_l$ being the corresponding street usage.
%
We take adaptive steps in the direction  $-\nabla E_{tot}(\{\mathbf{M}^{i,j}\})$ until the changes stabilize.

If necessary, we normalize the results to satisfy max and min travel time across the map boundaries. Note that, for this step, we only consider the energies that are continuous functions.
After each step, we adaptively check whether routes of the measured trips change without recomputing the paths from scratch. If they remain unchanged, we directly update the energy value; otherwise, we re-route as it is possible that other discrete functions may have different values. If total energy increases, usually because of the increase of the discrete energy, we ignore the change and the optimization switches back to topology optimization. % (annealing temperature is partially increased).


Figure~\ref{fig:global_opts_steps} shows a typical progression of this mixed optimization. Note that at the end of this stage, we only have the coarse connectivity along with corresponding target times (indicated by line thickness) for the active links. %Only in the next stage, the network is geometrically laid out, as explained next.


\begin{figure}[h!]
   \includegraphics[width=\columnwidth]{figures/algo_illustration/global_opt_stages.pdf}
   \caption{(Top)~Evolving connectivity matrices over iterations (150, 300, 450, respectively) of the global optimization.
   (Bottom)~Cumulative energy (Equation~\protect\ref{eq:optFunction}) against algorithm steps: blue segments of the curve denote improvements due to continuous optimization, while orange parts of the curve denote improvements due to discrete optimization. }
   \label{fig:global_opts_steps}
   \vnudge
\end{figure}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Local Geometry Layout}

We now describe how to geometrically realize a street layout corresponding to the coarse network designed in the previous stage. Note that at this stage we only have a coarse network in the form of connectivity matrices (across grid cell connectors) encoding connectivity and target travel times. We start by generating a candidate set of valid templates and then assigning the templates to the respective connectivity matrices $\{\mathbf{M}^{i,j}\}$. We cast the assignment process as a multi-label assignment problem, where candidate template labels are assigned based on how well they achieve the target travel time, while jointly considering neighboring labels to ensure connector continuity across adjacent grid cells.

%We first create a catalogue of valid template layouts using a simple procedure: We divide a grid cell boundary into $k \times k$ array ($k=3$ in our implementation) and test all possible connections with the links (i.e., street segment) turned either on or off. Note there are $2^{2k(k+1)}$ such combinations out of which many are ruled out as invalid (e.g., those with islands). We also support additional restrictions, e.g., discard templates with unnecessary loops, support dead ends. %All these will be checked to remove any invalid template layouts.
We first create a catalogue of valid template layouts using a simple procedure: We divide a grid cell boundary into $k \times k$ array ($k=6$ in our implementation) and test all possible connections with the links on the odd number lines (i.e., street segment) turned either on or off (links on the even number lines are always off). Note there are $2^{k(\frac{k}{2}+1)}$ such combinations out of which many are ruled out as invalid (e.g., those with islands). We also support additional restrictions, e.g., discard templates with unnecessary loops and dead ends. %All these will be checked to remove any invalid template layouts.
%
%For each connectivity matrix $\mathbf{M}$ (i.e., $\mathbf{M}^{i,j}$), say the candidate street templates are denoted as $\{T_{l}\}$ with corresponding compatibility scores $E_D(T_l, \mathbf{M})$ capturing how well the travel time in the template $T_l$ matches the target specification in the connectivity matrix.
For each connectivity matrix $\mathbf{M}$ (i.e., $\mathbf{M}^{i,j}$), we first classify the entries into four speed types (fast, middle, slow, and no connection). The candidate street templates are denoted as $\{T_{l}\}$ with corresponding compatibility scores $E_D(T_l, \mathbf{M})$ capturing how well the travel time in the template $T_l$ matches the target specification in the connectivity matrix speed type.
%
We estimate travel time for any $T_l$ among its connector points based on a modified Dijkstra's algorithm (see Figure~\ref{fig:local_templates}). In our implementation, we assume a fixed speed throughout the network, although one could consider location specific speeds in this stage.

\begin{figure}[t!]
  \includegraphics[width=\columnwidth]{figures/algo_illustration/local_steps1.pdf}
   \caption{In the local geometry layout stage, based on a $k\times k$ potential street layout~(left) we create various candidate template layouts~(right). We then select from these templates based on how well they conform to the global connectivity requirements $\{\mathbf{M}^{i,j}\}$ and agree with neighboring selected templates.
   }
   \label{fig:local_templates}
   \vnudge
\end{figure}


%In order to measure compatibility between any two templates $T_l$ and $T_m$, we simply measure the length of the extra street necessary to connect their corresponding contacts and encode it as  $E_C(T_l, T_m)$. Note that we take into consideration how the templates are to be connected (i.e., $T_l$ is to the left of $T_m$, etc.) in order to determine which connectors are to be linked. (We do not show this information in this notation.) For example, $E_C(T_l, T_m)=0$ when the active connectors match exactly across the shared boundary of the template.


%Now, given connectivity matrices $\{\mathbf{M}^{i,j}\}$, we pose a labeling problem using the Gibb's energy set as a combination of data (i.e., unary) terms as $E_D(T_l, \mathbf{M})$ and continuity (i.e., pairwise) terms as $E_C(T_l, T_m)$. We treat the labeling problem in the MRF setting and solve using $\alpha$-$\beta$ expansion.

We use a greedy algorithm to realize a geometric layout by assigning a template to each grid cell. For each cell, we randomly choose one of the templates that has best matching speed (since there can be multiple best candidates) and also agrees with existing neighboring selected templates. Since the number of valid templates is very large compared to the number of possible matrices $\mathbf{M}$, this simple solution works well in practice.

%Then we can measure a Euclidean distance from the template to a matrix catalogue. For the matrix catalogue, we classify each matrix to a catalogue by all entries value. We classify the entry's value into 4 groups: small, medium, large and no connection. Additionally, we can also category the templates by the enabled connectors on the sides.

%To replace cells of the grid with these templates, we do it in a random order. For each cell, we choose the template with the smallest distance and also satisfy the current connector constraint (which connector on the side is used for its neighbors). (So it's a simple greedy algorithm to decide the position of the connector on each side). For each cell, there are multiply candidates with same distances, and we randomly choose one.

Thus we only get the map of main skeleton of the street network. We can further add forks by grow road segments from each cell using a simple local strategy. For each cell, we grow the road network from the connectors, and randomly decide the order or whether have a new fork. However, for each iteration, we check whether the new road layout still satisfies the target matrix. Forks are allowed to grow into neighboring cells as long as it satisfy the connectivity matrices.
Loops can also be optionally created by growing road from the dead end to one of neighboring roads, as far as that will not create a shortcut of main skeleton.
In addition, we optionally allow the algorithm to detect and leave random blank spaces for relatively large parcels like parks or shops that are not pre-authored.

Finally, we remove any half road segment, i.e., a road segment to a connector is available on one cell's side but not available on the neighboring cell's side.



\begin{figure}[h!]
\centering
\includegraphics[width=0.42\columnwidth]{figures/usage/GridCell_parcel1}
\hfill
\includegraphics[width=0.42\columnwidth]{figures/usage/GridCell_parcel2}
   \caption{Left: a grid cell is further subdivided into smaller cells. Each cell is classified into one of four categories. Right: parcel layout with buildings.}
   \label{fig:parcel}
   \vnudge
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Parcel Generation}

The last stage of our pipeline is parcel generation. Parcel generation for a general configuration is a very difficult problem. Since we have multiple dead end streets, existing solutions~\cite{Vanegas:2012:PGO} are unable to compute parcel layouts for any of our street networks. To obtain a solution to the parceling problem, we make use of a simplifying assumption that parcels can be generated for each grid cell independently.
We use a rule-based approach for this purpose. Recall that in the previous step, a $k\times\,k$ array is created to further subdivide each grid cell for geometric realization. We can use the same array for parcel generation (see Figure~\ref{fig:parcel}). First, we classify the cells in the array into four types: (i)~a cell containing two street edges (cyan); (ii)~a cell containing one street edge (blue); (iii)~a cell containing one street vertex that is a dead end (green); and (iv)~a cell containing one street vertex that is a corner (pink). Second, each cell is split according to its type (See Figure~\ref{fig:parcel}).
We also implemented several post-processing heuristics to randomize parcel sizes, to merge parcels to generate larger parcels, and to generate and place buildings.


==> overview.tex <==
%\begin{figure*}[t!]
%\centering
%\includegraphics[width=1.0\linewidth]{figures/overview/pipeline}
%\caption{The pipeline of our approach. Starting from given boundaries (yellow), the street layout is generated in four levels in decreasing coverage ranges. For each level, we follow three main steps. First, a dense network of street segment candidates is generated in the form of a quad mesh. Second, a street layout is generated by selecting a subset of edges from the dense network using a mixed-integer programming approach (shown in grey). Third, the geometry of the generated street layout is smoothed (the last two levels are smoothed in one pass). The quad mesh is subdivided at the second and third levels for increased degrees-of-freedom. Dead ends are allowed only at the last level (e.g., cul-de-sacs). Due to computational costs, the first two levels are generated by the traffic-based model (Section~\ref{sec:traffic_based}) and the last two levels are generated by the coverage-based model (Section~\ref{sec:coverage_based}).}
%\label{fig:pipeline}
%\vnudge
%\end{figure*}

\section{Framework Overview}
\label{sec:overview}

Here, we provide an overview of our framework (see Figure~\ref{fig:pipeline}).

\mypara{Input specification.} We assume that the input problem domain, which presents an empty region of land, is given by surrounding (arterial) roads in the form of a 2D piece-wise linear polygon with zero or more holes.

\mypara{Multi-level street generation.} Inspired by the hierarchical nature of real-world street networks, we lay out the streets in multiple levels of decreasing traffic throughputs as follows.

\begin{enumerate}
\item We compute a dense network of street segment candidates in the form of a semi-regular (i.e., most vertices are of valence $4$) quadrilateral mesh, $M$, wherein the quads are roughly of uniform size and their shapes are close to a square. This assumption is based on the observation that real-world urban street layouts typically favor 90-degree intersections. In practice, the input problem domain is quadrangulated by the patch-wise quadrangulation algorithm in Peng et al.~\shortcite{Peng:2014:EQ:2577382.2541533}.
\item Beginning at the first level, an initial street layout is computed by selecting a subset of segments of the dense network. We formulate the problem as a mixed-integer programming (MIP) approach described in Section~\ref{sec:IP}.
\item The geometry of the street layout (i.e., positions of the vertices along the street edges) is further improved by a smoothing algorithm described in Section~\ref{sec:smoothing}. Afterwards, the remainder of the mesh is relaxed by standard Laplacian smoothing.
\item If the last level is not reached, we generate a dense network for the next lower level. To do so, we may need to increase the resolution of the mesh by a Catmull-Clark subdivision scheme without vertex repositioning for greater degrees of freedom of the MIP computation. The process starting with step 2 is then repeated at a lower level on the subdivided mesh.
\end{enumerate}


==> smoothing.tex <==
\begin{figure}[b!]
  % Requires \usepackage{graphicx}
  \centering
  \includegraphics[width=\columnwidth]{figures/smoothing/smoothing.pdf}
  \caption{Effects of different smoothing energies: (a) smoothing with all energies; (b) smoothing with a small tension energy; (c) smoothing without stiffness energy (thus the vertical white road at the T-junction in the middle is not smooth); (d) smoothing without inertia energy.}\label{fig:smoothing} \vnudge
\end{figure}

\section{Geometric Realization}
\label{sec:smoothing}

We describe how we geometrically realize the coarse street layout generated in the previous stage. The goal of this stage is to optimize the shape of the street layout to make it both visually realistic and functionally efficient. Note that in the previous stage, the generated street layout is a subset of the edges on a quadrilateral mesh. The geometry of the quad mesh is meant only for an approximation of the geometry of the actual street layouts. In particular, the layout may contain many sharp (90$^\circ$ degree angle) turns due to the nature of quadrilateral meshes. These sharp turns not only look unrealistic but also make the streets longer and more tenuous, e.g., stair-shaped, which leads to longer travel times.

We use the active contour model (snakes)~\cite{Kass:1988:SACM} to find the final shape of the street layout. In an active contour model, a snake is a spline guided by forces to minimize the associated energy for the purpose of geometrically smoothing it. We give a summary of the algorithm as follows.

A snake is a distinct non-empty sequence of present edges of the street layout that connects a distinct sequence of vertices (i.e., no branches nor loops). Moreover, the valence of the first and last vertices of a snake cannot be $2$; that is, a snake must end at non valence-$2$ vertices. A street layout is decomposed into snakes. It is straightforward to see that a layout can be decomposed into non-overlapping snakes that together fully cover the layout. Note that snakes can include intersection vertices of the street layout, i.e., a present vertex that connects to more than two present edges, from its interior. After the snakes are extracted, we subdivide each snake so that the smoothing algorithm, described next, may have a higher degrees of freedom.

The snake-based smoothing algorithm minimizes the energy associated with a deformable spline (a snake). In our setup, we consider three types of energies: tension, stiffness, and inertia. Assuming that a snake is represented by $\mathbf{u}(s, t)$, where $s \in (0, 1)$ is the parametric domain and $t$ is the time (i.e., iteration), for each vertex, the energies are defined as follows.

\begin{itemize}
  \item Tension energy, $E_\text{tension}(\mathbf{u})=\left| \frac{\partial \mathbf{u}(s)}{\partial s} \right|^2$. Minimizing the tension energy makes the snake act like a membrane. A higher weight for this energy leads to shorter lengths.
  \item Stiffness energy, $E_\text{stiffness}(\mathbf{u})=\left| \frac{\partial^2 \mathbf{u}(s)}{\partial^2 s} \right|^2$. Minimizing the stiffness energy makes the snake act like a thin plate. A higher weight for this energy leads to smoother turns.
  \item Inertia energy, $E_\text{inertia}(\mathbf{u})=\left| \mathbf{u}(s, t) - \mathbf{u}(s, 0) \right|^2$. This energy is used to prevent the snake from moving too far away from its original position.
\end{itemize}

The overall energy is defined as a linear combination of these three energies for all vertices:
\begin{equation}
E= \sum_\text{snake} \int_0^1 \left(\alpha E_\text{tension} + \beta E_\text{stiffness} + \gamma E_\text{inertia}\right) \mathrm{d}s.
\end{equation}
Here, $\alpha$, $\beta$, and $\gamma$ are the weights of the three energies.

We use different settings of weights at different levels of the street layout hierarchy. Streets at higher levels use higher stiffness weights (smoother corners) while streets at lower levels use higher inertia weights (fewer deformations). Additional heuristics are used to make sure the street intersections are close to 90$^\circ$ angles.

We use gradient descent to optimize the snake energy. The gradient of the snake energy is:
%
\begin{equation}
\begin{split}
\nabla E =\sum_\text{snake} \int_0^1 \bigg(-2\alpha \frac{\partial^2 \mathbf{u}(s)}{\partial s^2} + 2\beta \frac{\partial^4 \mathbf{u}(s)}{\partial s^4}+ \\
 2\gamma \left(\mathbf{u}(s, t) - \mathbf{u}(s, 0) \right) \bigg) \mathrm{d}s.
\end{split}
\end{equation}
We take adaptive steps in the direction of $-\nabla E$ until the changes stabilize.
